Far3D: Expanding the Horizon for Surround-view 3D Object Detection

Recently 3D object detection from surround-view images has made notable advancements with its low deployment cost. However, most works have primarily focused on close perception range while leaving long-range detection less explored. Expanding existing methods directly to cover long distances poses challenges such as heavy computation costs and unstable convergence. To address these limitations, this paper proposes a novel sparse query-based framework, dubbed Far3D. By utilizing high-quality 2D object priors, we generate 3D adaptive queries that complement the 3D global queries. To efficiently capture discriminative features across different views and scales for long-range objects, we introduce a perspective-aware aggregation module. Additionally, we propose a range-modulated 3D denoising approach to address query error propagation and mitigate convergence issues in long-range tasks. Significantly, Far3D demonstrates SoTA performance on the challenging Argoverse 2 dataset, covering a wide range of 150 meters, surpassing several LiDAR-based approaches. Meanwhile, Far3D exhibits superior performance compared to previous methods on the nuScenes dataset. The code is available at https://github.com/megvii-research/Far3D.

==> files/tmp.tex <==
% % intro figures
% \begin{figure}[t!]
%   \centering
%   \begin{subfigure}[b]{0.47\linewidth}
%     \includegraphics[width=\linewidth]{LaTeX/figures/intro_a.jpg} % Replace with the filename of your first subfigure
%     \caption{3D predicted boxes}
%     \label{fig:subfig1}
%   \end{subfigure}
%   % \hfill
%   \begin{subfigure}[b]{0.47\linewidth}
%     \includegraphics[width=\linewidth]{LaTeX/figures/intro_b.jpg} % Replace with the filename of your second subfigure
%     \caption{2D predicted boxes}
%     \label{fig:subfig2}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.9\linewidth}
%     \includegraphics[width=\linewidth]{LaTeX/figures/intro_c2.pdf} % Replace with the filename of your third subfigure
%     \caption{Recall comparisons in all ranges}
%     \label{fig:subfig3}
%   \end{subfigure}
%   \caption{Performance comparisons on Argoverse 2 between 3D detection and 2D detection. (a) and (b) demonstrate predicted boxes of Stream-PETR and YOLOX, respectively. (c) implies that 2D recall is notably better than 3D recall and can act as a bridge to achieve high-quality 3D detection.}
%   \label{fig:intro}
% \end{figure}

%% intro table recall
\begin{table}[t!]
    \centering
    \caption{Recall comparisons imply that 2D recall is notably better than 3D recall and can act as a bridge to achieve high-quality 3D detection.}
    \label{tab:intro_recall}
    \tiny
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Recall} & \textbf{0-50m} & \textbf{50-100m} & \textbf{100-150m} & \textbf{Average}      \\
    \toprule
    R@3D & 0.46 & 0.17 & 0.06 & 0.32 \\
    R@2D & 0.92& 0.68& 0.46 & 0.78 \\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> tables/av2_all_cls.tex <==
\begin{table*}[th!]
\centering
\caption{Performance of most categories in Arogverse 2 \texttt{val} set. The metric is mAP\%.}
\label{tab:av2_all_cls}
\tiny
\resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l|ccccccccccccccccccccc}

\toprule
\textbf{Methods} & \rotatebox{60}{Average} & \rotatebox{60}{Vehicle}  & \rotatebox{60}{Bus} & \rotatebox{60}{Pedestrian} & \rotatebox{60}{Stop Sign} & \rotatebox{60}{Box Truck} & \rotatebox{60}{Bollard} & \rotatebox{60}{C-Barrel} & \rotatebox{60}{Motorcyclist} & \rotatebox{60}{MPC-Sign} & \rotatebox{60}{Motorcycle} & \rotatebox{60}{Bicycle} & \rotatebox{60}{A-Bus} & \rotatebox{60}{School Bus} & \rotatebox{60}{Truck Cab} & \rotatebox{60}{C-Cone} & \rotatebox{60}{V-Trailer} & \rotatebox{60}{Sign} & \rotatebox{60}{Large Vehicle} & \rotatebox{60}{Stroller} & \rotatebox{60}{Bicyclist} 
\\
% 22.0 67.6 38.9 46.5 16.9 37.4 40.1 32.2 28.6 27.4 33.4 24.5 8.7 25.8 22.6 29.5 22.4 6.3 3.9 0.5 20.1 
% 28.2 68.1 40.9 59.0 29.0 38.5 41.8 42.6 39.7 26.2 49.0 38.6 20.4 30.5 14.8 41.2 26.9 11.9 5.9 13.8 33.4 
% 30.0 71.7 39.2 63.1 39.2 40.0 52.5 63.7 42.2 34.9 42.7 40.1 20.1 25.2 16.9 45.7 22.3 15.8 5.9 9.8 33.5 
% 30.7 72.7 38.8 63.2 40.2 40.1 53.9 64.9 44.7 39.4 42.4 40.6 20.1 25.2 19.9 44.9 20.9 14.9 6.8 15.7 32.4 
\midrule
% CenterPoint~\cite{yin2021center} & 22.0 &  67.6 &  38.9 &  46.5 &  16.9 &  37.4 &  40.1 &  32.2 &  28.6 &  27.4 &  33.4 &  24.5 &  8.7 &  25.8 &  22.6 &  29.5 &  22.4 &  6.3 &  3.9 &  0.5 &  20.1 \\ 
FSD & 28.2 & 68.1 & 40.9 & 59.0 & 29.0 & 38.5 & 41.8 & 42.6 & 39.7 & 26.2 & 49.0 & 38.6 & 20.4 & 30.5 & 14.8 & 41.2 & 26.9 & 11.9 & 5.9 & 13.8 & 33.4 \\ % ~\cite{fan2022fully}
VoxelNeXt & 30.7 & 72.7 & 38.8 & 63.2 & 40.2 & 40.1 & 53.9 & 64.9 & 44.7 & 39.4 & 42.4 & 40.6 & 20.1 & 25.2 & 19.9 & 44.9 & 20.9 & 14.9 & 6.8 & 15.7 & 32.4 \\ % ~\cite{chen2023voxelnext}
\rowcolor[gray]{.9} 
Ours & 30.7 & 52.4 & 34.4 & 37.6 & 36.5 & 24.3 & 36.6 & 44.3 & 43.7 & 35.7 & 52.0 & 40.0 & 25.1 & 31.9 & 23.9 & 52.5 & 22.7 & 20.8 & 5.1 & 33.6 & 25.0 \\

\bottomrule
\end{tabular}
}
% \vspace{-0.25cm}
\end{table*}

==> tables/nus_test_set.tex <==
\begin{table*}[th!]
\centering
\caption{Comparison on the nuScenes \texttt{test} set.}
\vspace{-0.2cm}
\label{tab:nus_test_set}
\tiny
\resizebox{0.95\textwidth}{!}{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l|c|c|cc|ccccc}

\toprule
\textbf{Methods} & \textbf{Backbone} & \textbf{Image Size}  & \textbf{mAP}$\uparrow$  &\textbf{NDS}$\uparrow$  & \textbf{mATE}$\downarrow$ & \textbf{mASE}$\downarrow$   &\textbf{mAOE}$\downarrow$ &\textbf{mAVE}$\downarrow$   &\textbf{mAAE}$\downarrow$\\
\midrule
% ResNet50 256 x 704
SOLOFusion & ConvNeXt-B & 640 $\times$ 1600
& 0.540 & 0.619 & 0.453 & 0.257 & 0.376 & 0.267 & 0.148 \\ 
Sparse4Dv2 & VoV-99 & 640 $\times$ 1600
& 0.556 & 0.638 & 0.462 & 0.238 & 0.328 & 0.264 & \textbf{0.115}\\ 
StreamPETR & ViT-L & 800 $\times$ 1600
& 0.620 & 0.676 &0.470  &0.241  & \textbf{0.258}  & 0.236  &0.134\\ 
\rowcolor[gray]{.9} 
\far{}~(Ours)  &  ViT-L & 800 $\times$ 1600
& \textbf{0.635} & \textbf{0.687} & \textbf{0.432} & \textbf{0.237} & 0.278 & \textbf{0.227} & 0.130 \\ 
% Ours & ResNet101 & 512 $\times$ 1048
% & & & &  &  & &   \\ 
\bottomrule
\end{tabular}}
% \vspace{-0.25cm}
\end{table*}
